Multiple Source Dual Fault Tolerant BFS Trees

Let $G=(V,E)$ be a graph with $n$ vertices and $m$ edges, with a designated set of $\sigma$ sources $S\subseteq V$. The fault tolerant subgraph for any graph problem maintains a sparse subgraph $H$ of $G$, such that for any set $F$ of $k$ failures, the solution for the graph problem on $G\setminus F$ is maintained in $H\setminus F$. We address the problem of maintaining a fault tolerant subgraph for Breath First Search tree (BFS) of the graph from a single source $s\in V$ (referred as $k$ FT-BFS) or multiple sources $S\subseteq V$ (referred as $k$ FT-MBFS). The problem of $k$ FT-BFS was first studied by Parter and Peleg [ESA13]. They designed an algorithm to compute FT-BFS subgraph of size $O(n^{3/2})$. Further, they showed how their algorithm can be easily extended to FT-MBFS requiring $O(\sigma^{1/2}n^{3/2})$ space. They also presented matching lower bounds for these results. The result was later extended to solve dual FT-BFS by Parter [PODC15] requiring $O(n^{5/3})$ space, again with matching lower bounds. However, their result was limited to only edge failures in undirected graphs and involved very complex analysis. Moreover, their solution doesn't seems to be directly extendible for dual FT-MBFS problem. We present a similar algorithm to solve dual FT-BFS problem with a much simpler analysis. Moreover, our algorithm also works for vertex failures and directed graphs, and can be easily extended to handle dual FT-MBFS problem, matching the lower bound of $O(\sigma^{1/3}n^{5/3})$ space described by Parter [PODC15].The key difference in our approach is a much simpler classification of path interactions which formed the basis of the analysis by Parter [PODC15]. Our dual FT-MBFS structure also seamlessly gives a dual fault tolerant spanner with additive stretch of +2 having size $O(n^{7/8})$.

==> algo.tex <==
\section{Implementation of Dual FT-MBFS algorithm}
\label{appn:algo}
%%%%%%%%%%%% MOVE TO INTRO
%We shall now formally introduce the problem.
%Given an unweighted graph $G=(V,E)$ and a source vertex $s\in V$, the aim is to compute a
%sparse unweighted graph $H=(V,E')$ with $E'\subseteq E$ which satisfies the following property.
%For any failure of $F\in E$ (where $|F|\leq 2$), the length shortest path between $s$ and any $v\in V$
%in $G\setminus\{F\}$ is equal to the length of shortest paths between $s$ and $v$ in $H\setminus\{F\}$.
%Algorithm~\ref{alg:dual_BFS} computes this sparse graph $H$ for a given source $s\in V$.
%Note that our algorithm is similar to the one presented by \cite{Parter15} with a different analysis.
%Further, our space analysis is much simpler and hence extendible to handle multiple sources as well.
%%%%%%%%%%%%%%%%
We shall now describe the implementation details of our algorithm to compute sparse 
dual FT-MBFS subgraph $H$ from a set of $\sigma$ sources $S\subseteq V$.
For every vertex $v\in V$, our algorithm computes the shortest paths from each $s\in S$ to $v$
avoiding upto two failures and adds the last edge of each such path to the adjacency list of vertex $v$. 
Note that repeating the procedure for each vertex on such a path adds the entire path to $H$ 
\cite{ParterP13,Parter15}.

%We first order the edges on any failure $F$ in order $\{e_1,e_2\}$ as follows.
%For any $i=1,2$ in order, we assign the edge $e_i$ to be the highest edge on $P_{i-1}$ from $F$.
%Note that in case of $i=2$, $\{e_1\}$ have already been assigned hence we have a corresponding $P_{i-1}=P_1$.
%In case the remaining edges (not assigned as any $e_j$, for $j<i$) do not lie on $P_{i-1}$,
%we simply ignore them and report the shortest path $P_{i-1}$ for the entire $F$.

Our algorithm starts by adding the shortest path between $s$ and $v$, i.e., $P_0$. It then processes single edge failures on $P_0$. We then find the replacement path  $P$ for all two edge failures $\{e_1, e_2\}$ such that $e_1 \in P_0$ and $e_2 \in P_1$. Further, in case $e_2\in P_0\cap P_1$
then $e_1$ is higher than $e_2$ on $P_0$.

However, we want to process all the failures  in some particular order. This ordering plays a crucial role in the analysis. To this end, we define this ordering $\pi$  as follows. The first failure  in $\pi$ is $F = \emptyset$, which adds $P_0$. The ordering $\pi$ then contains single edge failures of type  $F=\{e\}$ (where $e\in P_0$),
ordered by their decreasing distance from $s$ on $P_0$.
 Finally, we order the remaining failures as follows: for any two failures $F=\{e_1,e_2\}$ and $F'=\{e'_1,e'_2\}$ (with corresponding replacement paths $P$ and $P'$), $F\prec_{\pi} F'$ if either (1) $e_1$ is farther than $e_1'$ from $s$ on $P_0$, or (2) $e_1 = e_1'$ and $e_2$ is farther than $e_2'$ from $s$ on $P_1$ (note that $P_1 = P_1'$ in this case). If $F\prec_{\pi} F'$, $F$ is said to be {\em lower} than $F'$
in $\pi$.



For any failure of $F = \{e_1,\cdots,e_k\}$, we define the {\em preferred}  shortest path avoiding $F$. 
Our preferred shortest path will be a path of shortest length avoiding $F$. However, there can be 
multiple such paths of same length. We use  following rules to choose a unique preferred path.
%These seemingly unintuitive restrictions play a crucial role in the space analysis of our algorithm.
\begin{definition}
Path $P$ is \textbf{preferred} for failure of $\{e_1,\cdots,e_k\}$ where each $e_i\in P_{i-1}$, if
\begin{enumerate}
        \item For each $i$, $P$ leaves $\Pth{}{i-1}$ before $e_i$ exactly once.
        \item For any other $P'$ also avoiding $\{e_1,\cdots,e_i\}$, we have either
        (i) $|P|<|P'|$, 
        (ii) $|P|=|P'|$, and for some $0\leq i\leq k$, both $P$ and $P'$ leaves each of 
        $P_0,...,P_{i-1}$ at the same vertex, but $P$ leaves $P_i$ earlier than $P'$,
        (iii) $P$ is lexicographically smaller
        \footnote{
% If we give each vertex a unique alphabet from an totally ordered universe \small{$\sum$}, then $P$ is
%lexicographically shorter than $P'$ if the vertex where $P$ and $P'$ differ satisfy.
Let $P$ and $P'$ first diverge from each other to $x \in P$ and $x' \in P'$ respectively, i.e.,
$P[s,x]\setminus \{x\}=P'[s,x']\setminus \{x'\}$. If the index of $x$ is lower than
that of $x'$ then $P$ is said to be {\em lexicographically smaller} than $P'$.} than $P'$.
%       the index of the first point of divergence
%       of $P$ and $P'$ is lower in $P$ than in $P'$
%       of distinction is lower in $P$ $P[x,x]=P'[s,x]$.
\end{enumerate}
\end{definition}
%%%%%%%%%%%%%%%%%%%          IMP NOTE
%% ADD SIGNIFICANCE OF leaving $\Pth{}{0}$ and $\Pth{}{1}$
%%%%%%%%%%%%%%%%%%%%%%%

Intuitively, out of all the shortest paths avoiding $F$ (say for $|F|=2$), 
the preferred path leaves the  path $P_0$ and/or $P_1$
as early as possible. In order to avoid the preferred path leaving $P_0$ (or $P_1$) multiple
times just to achieve an earlier point of divergence from $P_0$ (or $P_1$),
the first condition is imposed. The last condition in (2) is just to break ties
between two paths that are of same length and leave $P_0$ and $P_1$ at the same vertex.




Finally, in order to add the preferred shortest path $P$ avoiding a failure $F$,
our algorithm simply adds $\LE(P)$ to $H$, which suffices to add the entire path as
described earlier.
Moreover, we also assign the corresponding $P$ to the failure $F$
if it was the first failure to add this edge in $H$. 
As a result if $P,P'$ are two preferred paths
avoiding $F$ and $F'$ respectively where $\LE(P)=\LE(P')$, 
the path $P$ shall be assigned to $F$ if $F\prec_{\pi} F'$. 
%As a result if $P,P'$ are two preferred paths
%avoiding $\FT(P)$ and $\FT(P')$ with $\LE(P)=\LE(P')$, the path $P$
%shall be assigned to $\FT(P)$ if $\FT(P)\prec_{\pi} \FT(P')$. 
Refer to Procedure~\ref{alg:dual_BFS} for the
pseudocode of our algorithm.\\
        \begin{procedure}[H]


                   \ForEach{Failure $F$, where $0\leq |F|\leq 2$, ordered from lower to higher in $\pi$}
                        {
                                $P\leftarrow$ {\em Preferred} path from $s$ to $v$ in $G$ avoiding $F$\;
                                \If{$\LE(P)\notin H$}
                                {
                                        Assign $P$ for failure of $F$\;
                                        Add $\LE(P)$ to $H$\;
                                }
                        }
                \caption{Dual-FT-BFS($s,v,\pi$):
                        Augments the dual FT-BFS subgraph $H$, such that for BFS tree of $G$ rooted at $s$ 
                        after any two edge failures in $G$, the incoming edges to $v$ are preserved in $H$.                       
%                        Creates a subgraph $H$ which preserves the BFS tree of $G$ rooted at $s$
%                        after any two edge failures in $G$.
                }
                \label{alg:BFS}
        \end{procedure}


Given a source $s$, let $\pi_s\subseteq \pi$ denote the ordering of edge failure of size upto 2.
Let $\pi_s(0), \pi_s(1)$ and $\pi_s(2)$ be the subset of $\pi_s$ of size 0, 1 and 2 respectively. 
Our algorithm for finding dual FT-MBFS mimics the single source case.

%\begin{wrapfigure}[7]{l}{0.6\textwidth}

        \begin{procedure}[H]
                        \LinesNotNumbered
                \lForEach{$s \in S$}
                {
                    Dual-FT-BFS($s$,$v$,$\pi_s(0)$)
                }
                \lForEach{$s \in S$}
                {
                    Dual-FT-BFS($s$,$v$,$\pi_s(1)$)
                }
                \lForEach{$s \in S$}
                {
                    Dual-FT-BFS($s$,$v$,$\pi_s(2)$)
                }
                \caption{Dual-FT-MBFS($S$,$v$,$\pi$):
                                Augments the dual FT-MBFS subgraph $H$, such that for BFS tree of $G$ rooted at each $s\in S$
                after any two edge failures in $G$, the incoming edges to $v$ are preserved in $H$.
%                Creates a subgraph $H$ which preserves the BFS tree of $G$
%                rooted at sources in $S$ after any two edge failures in $G$.
                }
                \label{alg:MBFS}
        \end{procedure}
%\end{wrapfigure}

The first for loop in the above procedure finds shortest path from each source to $v.$
We shall refer to the set of the shortest paths from each source to $v$ for different $s\in S$
as $\PP_0$. We then move on to find the shortest path from each source to $v$ avoiding one edge failure and two failures respectively.


==> dualFDirectedPd.tex <==
Our analysis of dual FT-BFS for undirected graphs extends to the directed case, 
except the case of short standard paths $\PP_c$. 
The exact problem occurs when we use $LL(P)[y',y]$ when finding
an alternate path in Section \ref{sec:pc}. While using this path, we crucially
use the fact that the graph is undirected. Unfortunately, if the graph is directed,
we cannot use this path. So, in this section, we give a different analysis for $\PP_c$.
We shall first define the notion of a {\em segmentable} paths 
(similar to the notion of {\em regions} used by Parter~\cite{Parter15})
and describe its properties as follows.


\begin{definition} We define the following terms for any set of shortest paths $\Ps$ and $\Ps_*$
        to the vertex $v$,  where any $P\in \Ps$ is the shortest path from $\SC(P_*)$ avoiding failure
        of some edge $e\in P_*$ for some $P_*\in \Ps_*$.
        %Moreover, except for $e$, $P$ can traverse any edge on a path in $\Ps\cup \Ps_*$.
        Also, let $\DE_*(P)$ be the detour of $P\in\Ps$ from corresponding $P_*\in \Ps_*$.
        %Let $Dest(P^*)=d^*$ be the last vertex in $P^*$
        \begin{itemize}
        \item \textbf{Segmentable Paths:}
        The set of paths $\Ps_*$ is called segmentable if $\Ps_*$ is converging.
%        The set of paths $\Ps_*$ is called as segmentable if any two paths in $\Ps_*$ intersects,
%        they do not diverge after the point of intersection.
        \item \textbf{Segments of $\Ps_*$:}
        If any path $P_*\in \Ps_*$ intersects with other paths in $\Ps_*$ on vertices $x$ and $y$,
        the path $P_*[x,y]$ is called a {\em segment} of $\Ps_*$ if it does not intersect any path of
        $\Ps_*$ except at its endpoints. The segment of $\Ps_*$ from which $\DE_*(P)$ of some $P\in \Ps$
        emerges from the corresponding $P_*\in \Ps_*$ is represented by $P_s$.
        \item \textbf{Representatives of a segment:} For any segment $P_s=P_*[x,y]$, the shortest
        path from $x$ to $v$ avoiding $P_*[y,v]$ is called the {\em representative path} of $P_s$,
        and is denoted by $R_s$. Also, the last vertex of $R_s$ on $P_s\cap R_s$, say $v_{s^*}$,
        is called the {\em representative vertex} of $R_s$. %, and is denoted by $v_{s^*}$.
        \end{itemize}
        \label{def:seg-paths}
\end{definition}

The properties of a {\em segmentable} paths can be described as follows.
\begin{lemma}
        The segments of a set of segmentable paths $\Ps_*$ have the following properties.
   \begin{enumerate}
   \item Number of segments of $\Ps_*$ are $2|\Ps_*|$.
   \item For any path $P'\in\Ps$ following the representative path of some segment $P_s$,
                 $P'[v_{s^*},v]=R_s[v_{s^*},v]$.
%   Number of paths in $\Ps$ that follow the representative paths of some segment
%                are $2|\Ps_*|$.
   \item For any paths $P,P'\in\Ps$ that diverge from segment $P_s=P_*[x,y]$ and
                  $P'_s=P'_*[x',y']$ respectively, if $P$ and $P'$ do not follow any path in $\Ps_*$
                  or representative path of any segment in $\Ps_*$, say set of such paths is $\Ps'$, we have
                \begin{enumerate}
                        \item $e\in P_s[x,v_{s^*}]$.
                        \item $\DE_*(P)$ does not intersect with $P'_s[x',v'_{s^*}]$ if $P'_s\neq P_s$.
                        \item The set of paths $\{\DE_*(P)|P\in \Ps'\}$ is converging.
%                        \item $\DE_*(P)$ and $\DE_*(P')$ do not diverge after intersecting with each other
%                        (if they intersect).
                \end{enumerate}
   \end{enumerate}
        \label{lem:seg-prop}
\end{lemma}
\begin{proof}
\begin{enumerate}
\item By definition of {\em segmentable} paths, whenever two or more paths $P_*$ and $P'_*$
 intersect they merge to form a single path. Thus, each $P_*$ originates from a unique vertex.
Also, since on intersection of two or more such paths they merge to form a single path,
the number of paths reduces by at least one after the intersection. This limits the total number of
intersection points among the paths in $\Ps_*$ to $|\Ps_*|$. Now, each segment can be uniquely associated
with starting vertex which can be a source of corresponding path in $\Ps_*$ or an intersection point described above.
Hence, we have only $2|\Ps_*|$ segments.

\item Now, for the segment $P_s=P_*[x,y]$, the representative path is the shortest path avoiding
 $P_*[y,v]$. Hence, any path $P'$ which follows the representative path leaving $P_s$ necessarily
 has $e'\in P_*[v_{s^*},v]$. Since $R_s$ avoids entire $P_*[v_{s^*},v]$ (containing $e$) and
$P'$ is not required to avoid any other edge in $\Ps\cup\Ps_*$, $P'$ will not diverge from $R_s$ after $v_{s^*}$.
Hence, we have $P'[v_{s^*},v]=R_s[v_{s^*},v]$.
%Thus, at most one contributing path can follow each
%representative path of some segment of $\Ps_*$, limiting the number of such paths to
%$2|\Ps_*|$.

\item Finally, consider the case when a path $P$ does not follow the representative path of any segment of $\Ps_*$.
\begin{enumerate}
\item %Since $R_s$  is the shortest path avoiding $P_*[y,v]$,  $P$ has to leave $P_s$ before $v_{s^*}$.
%This is possible only if $e_2\in P_s[x,v_{s^*}]$, else $P$ would clearly follow $R_s$.
Since $P$ leaves the segment $P_s$, unless $e\in R_s$ it would follow the shortest path
avoiding $P_*[y,v]$ (i.e. $R_s$). Also, by definition $e\in P_*$, hence  $e\in P_*\cap R_s=P_s[x,v_{s^*}]$.
\item We shall prove this by contradiction. Hence, let $P'_s$ be the last segment to which
$\DE_*(P)$ intersects in the corresponding $P'_s[x',v'_{s^*}]$.
Clearly, $P$ diverges from $P'_s$ else it would intersect the next segment $P''_s$ at $x''$ (where $y'=x''$)
if $P''_s$ exists, otherwise if $P'_s$ is the last segment $P$ will follow the corresponding path $P'_*\in \Ps_*$.
Both these cases contradicts our assumption, ensuring $P$ diverges from $P'_s$.
Since $e\in P_s$ and $P_s\neq P'_s$, we surely have $e\notin P'_s$.
Since $P$ diverges from $P'_*$ and $e\notin P'_s$ (as $e\in P_s\neq P'_s$), we have $e\in P'_*[y',v]$.
%Since $\DE_*(P)$ cannot intersect $P_s$ (using $\Prop_2$) and $e\in P_s$, we surely have $e\notin P'_s$.
%Further, since $P$ diverges from $P'_*$ with we have $e\in P'_*[y',v]$ (as $e\notin P'_s$).
This ensures $e\notin P'_{s^*}$ as it avoids the entire path $P'_*[y',v]$.
Since $P$ intersects $P'_*[x',v'_{s^*}]$ and avoids $P'_*[y,v]$, it will follow the shortest path
avoiding $P'_*[y',v]$, i.e. the representative path $P'_{s^*}$ as $e\notin P'_{s^*}$.
This contradicts our assumption and hence proves our claim.
\item Again, we shall prove this by contradiction. Assume $w$ is the last vertex at which
$\DE_*(P)$  intersects  $\DE_*(P')$ after which they diverge. Without loss of generality
assume $|P[w,v]|\leq |P'[w,v]|$. Now, since $P'$ diverges from $P$, i.e., avoids $P[w,v]$ which
implies $e'\in P[w,v]$ (as $w\neq v$). Further, using  3(a)
and 3(b), we know that $e\in P'_s[x',v'_{s^*}]$ whereas $\DE_*(P)$ cannot intersect with any
$P'_s[x',v'_{s^*}]$. Thus, we have $e'\notin P[w,v]$ disproving our assumption and proving
our claim.
\end{enumerate}
\end{enumerate}
\end{proof}


\subsection{Analyzing short standard paths $\PP_c$ for dual FT-BFS}
Using Lemma~\ref{lem:stdpath-prop}\ref{lem:detourC-Interleave}, we know that 
the set of $\{\DE_0(P_1) | P_1 \in \PP_{1c} \}$ forms a set of segmentable paths ($\Ps_*$).
Since we consider only those paths
in $\PP_c$ which emerge from $\DE_0(P_1)$ (using Lemma~~\ref{lem:lastP-Prop}\ref{lem:lastP-long}),
the set of paths $\DE_0(P)$ for $P\in \PP_c$ starts from the same vertex as the corresponding $\DE_0(P_1)$.
Also, by definition of {\em standard paths}, $\DE_0(P_1)$ does not intersect with $P_{high}$ and $e_1\in P_{high}$.
Thus, $\DE_0(P)$ is the shortest path from $\SC(\DE_0(P_1))$ to $v$ avoiding $e_2\in \DE_0(P_1)$.
Hence, for all $P\in \PP_c$, we can apply Lemma~\ref{lem:seg-prop} using $\Ps_*$ as the set $\{\DE_0(P_1) | P_1 \in \PP_{1c} \}$,
$\Ps$ as the set $\{\DE_0(P) | P \in \PP_c \}$, $\DE_*(P)$ as $\DE_1(P)$, and $e\in P_*$ as the corresponding $e_2\in P_1$.

%Now, we shall first prove that for the paths in $\PP_{1c}$, the set of $\DE_0(P_1)$ forms a set of
%segmentable paths. Using Lemma~\ref{lem:detourC-Interleave}, we know that any two such paths cannot
%diverge after intersecting. Further, we are required to prove that for any paths $P,P'\in \PP_c$,
%$e_1\notin \DE_0(P'_1)\cup \DE_0{P'}$ (see Definition~\ref{def:seg-paths}).
%By definition of $\PP_c$, $\DE_0(P'_1)$ merges with $P_0$ on $P_{low}$ whereas $e_1\in P_{high}$.
%Further, since we need to consider only the paths in $\PP_c$ which emerge from $\DE_0(P_1)$ (using Lemma~\ref{lem:lastP-long}), the corresponding $\Ps$ would correspond to $\DE_0{P'}$ covering all the such paths in $\PP_c$.
%Using $\Prop_2$ we clearly have $\DE_0(P')$ does not intersect with $P_0$ and hence $e_1\notin \DE_0(P')$.
%Hence, the set of paths in $\DE_0(P_1)$ forms a set of segmentable paths ($\Ps_1$),
%for $P_1\in \PP_{1c}$ with the corresponding $\Ps$ being the all the paths in $\PP_c$ which emerge from $\DE_0(P_1)$.

Now, by definition every path in $\Pthr{\PP}{1}{c}$ we have $|\DE_0(P_1)|\leq n^{2/3}$.
Thus, the total number of paths in $\DE_0(P_1)$ for all $P_1\in \PP_{1c}$ are $O(n^{2/3})$.
This also limits the number of segments of $\DE_0(P_1)$ to $O(n^{2/3})$ (using Lemma~\ref{lem:seg-prop} (1)).
Since, two contributing paths enter $v$ using a unique edge, using Lemma~\ref{lem:seg-prop} (2) there will
be exactly one path in $\PP_c$ that follows the representative path of each segment,
and none that follow any path in $\PP_{1c}$
%contributing path in $\PP_{1c}$ does not follow any path in $\PP_{1c}$
(else such paths are non-contributing). Thus the number of
paths in $\PP_c$ that follow the representative path or a path in $\PP_{1c}$ is limited to $O(n^{2/3})$.
Now, except for these $O(n^{2/3})$ paths, any two paths in $P,P'\in\PP_c$ also satisfies that
$\DE_1(P)$ and $\DE_1(P')$ do not diverge if they intersect (using Lemma~\ref{lem:seg-prop}~3(c)).
Since, each path in $\PP_c$ is contributing it hence enter $v$ from a unique edge,
its $\DE_1(P)$ cannot intersect with detour of any other path in $\PP_c$.
The number of such paths with $|\DE_1(P)|> n^{1/3}$, can clearly by restricted to
$O(n^{2/3})$. Hence, for the remaining paths in $\PP_c$ we have $|\DE_1(P)|<n^{1/3}$ giving the following corollary.

\begin{lemma}
Except for $O(n^{2/3})$ paths in $\PP_c$, for any paths  $P\in\PP_c$ we have  $|\DE_1(P)|\leq n^{1/3}$.
\label{lem:Pd-short-detour}
\end{lemma}


We shall now bound the number of paths in $\PP_c$ to $O(n^{2/3})$.
Let $\PP'_c$ be the set of paths in $\PP_c$ removing $O(n^{2/3})$ paths described in Lemma~\ref{lem:ms-Pd-P1-prop}.
Also, let $\PP'_{1c}$ be the corresponding $P_1$ for each $P\in \PP'_c$.
Thus, for any path $P\in \PP'_c$ we have $|\DE_1(P)|\leq n^{1/3}$ and $|\DE_0(P_1)|<n^{2/3}$ (by definition of $\PP_c$).
Further, for any path $P\in \PP_c$ we have $|P|\geq |P_0|$ (since $P$ is a detour from $P_0$).
Let $x=\SC(\DE_0(P_1))$ and $y=\SC(\DE_1(P))$.
Thus, any path $P\in \PP'_c$ can be divided into three parts  as follows.
\begin{align*}
        |P|     &=              |P[s,x]|+|P[x,y]|+|P[y,v]|\\
                        &=   |P_0[s,x]|+|\DE_0(P_1)[x,y]|+|\DE_1(P)[y,v]| &\qquad\text{(by definition of $x$ and $y$)}\\
                        &\leq   |P_0|+|\DE_0(P_1)|+|\DE_1(P)|\leq |P_0[s,v]|+n^{2/3}+n^{1/3}
\end{align*}

Using Lemma~\ref{lem:stdpath-prop}\ref{lem:diffP}, we know that for any $P,P'\in \PP_c$ we have $|P|\neq |P'|$.
We thus arrange the paths in $\PP'_c$ in the increasing order of sizes,
where $i^{th}$ such path has the length $\geq |P_0|+i$.
Since for any $P\in \PP'_c$ we also have  $|P|\leq |P_0|+2n^{2/3}$,
clearly the number of paths in $\PP'_c$ (and hence $\PP_c$) are $O(n^{2/3})$.
%Thus, we have the following theorem.
%
%\begin{theorem}
%        The number of contributing paths of the type $\PP_c$ are $O(n^{2/3})$ for dual FT-BFS on directed graphs.
%        \label{thm:contPdD}
%\end{theorem}


==> ms-dualFDirectedPd.tex <==
\subsection{Analyzing short standard paths $\PP_c$ for dual FT-MBFS }
Like the single source case, we want to bound the number of contributing paths in $\PP_c$ using segmentable paths. We first take case of all the paths $P$ with $\DE_0(P_1) \ge n_\sigma^{2/3}$ as follows.

Using Lemma~\ref{lem:ms-p0-Interleave}, we know that $\PP_0$ and hence $\Ps_{high}$ is a set of segmentable paths.
Moreover, each $P_1\in \PP_{1c}$ is the shortest path to $v$ avoiding $e_1\in \Ps_{high}$.
Thus, for any $P_1\in \PP_{1c}$, $\DE_0(P_1)$ emerges from $\Ps_{high}$ and merges back to some $P_0\in \Ps_{low}$.
Hence, we can use Lemma~\ref{lem:seg-prop} using $\Ps_*$ as $\Ps_{high}$,
$\Ps$ as $\PP_{1c}$, $\DE_*(P)$ as $\DE_0(P_1)$, and $e\in P_*$ as the corresponding $e_1\in P_0$.
Note that by definition, the representative path of $P_s=P_*[x,y]$, that is $R_s$, avoids $P_*[y,v]$
where $P_* \in \Ps_{high}$. Note that $P_*$ is actually a path from some source $s$ to $v$ till $v_{ls}$.
Thus, $P_*[y,v]$ exists and our definition of representative path is still valid.

Consider any segment $P_s \in P_0$.
Using  Lemma~\ref{lem:seg-prop} (2), we claim that once a  path in $P_1' \in \PP_{1c}$
intersect $P_s$ and follow representative path of $P_s$\ (i.e., $R_s$),
then it  cannot diverge from $R_s$.
%This is because if some $P_1' \in \PP_{1d}$ diverge from $P_s$ and  $R_s$
%(at a vertex, say $x$), it necessarily implies (1) $e_1'\in P_0$  and (2)$e_1' \in R_s[x,v]$.
%But $e_1' \in \Ps_{high}$ and by definition the representative path of $P_s$ avoids subpath of
%$P_0$ that lies in $\Ps_{high}$.
Using Lemma \ref{lem:ms-stdpath-prop}(\ref{lem:ms-LP-nonLL0}), for each such $P_1'$, we are concerned with those
$P' \in \PP_c$, that starts from $\MD{P_1'}$. We now claim that $\MD{P_1'}$
lies on $R_s$. This is due to the fact that both these paths are same
from the segment $P_s$.
We can easily bound the number of paths in $\PP_c$, that
starts from $R_s$. Let $\PP_e$ denote the set of these paths.
Since $\PP_e \subset \PP_c$, Lemma \ref{lem:ms-contProp} applies on all the paths in $\PP_e$.
We will now bound $\PP_e$ in a way similar to $\PP_a$.
Using Lemma \ref{lem:lastP-Prop}($c^*$), all the paths in $P \in \PP_e$ with $\LL(P) \ge n_\sigma^{1/3}$
can be bounded to $O( \sigma^{1/3}n^{2/3})$. For the rest of the paths, their last path
 have length $\le n_\sigma^{1/3}$, thus they necessarily starts on the lowest
 $n_\sigma^{1/3}$ vertices of representative paths.
%Thus, we can shift our focus from these $P_1' \in \PP_{1d}$
%to the representative path $R_s$ and try to analyze contributing paths $P' \in \PP_d$
%that start from $\MD_{R_s}$.
Using Lemma~\ref{lem:seg-prop} (1), since $|\PP_0|=\sigma$,
there are at most $2\sigma$ representative paths. Thus the total number of path $P \in \PP_e$
with small last paths is $O(\sigma n_\sigma^{1/3}) = O( \sigma^{1/3}n^{2/3})$.

Consider a path $P_1' \in \PP_{1c}$ that follows $P^* \in \Ps_{high}$ but not any representative path.  However, such path are non-standard paths (as $P_1'$ merges at $\Ps_{high}$). So, paths which follow $P^* \in \PP_{1c}$ do not exist in $\PP_{1c}$.

For the remaining
%Hence, the number of paths in $\PP_{1d}$ which follow the representative path of some segment
%of $\PP_0$ would be $|\PP_0|=\sigma$ (using Lemma~\ref{lem:seg-prop} 3(b)). For the remaining
paths $P_1,P'_1\in \PP_{1c}$ (that donot follow any representative paths and donot follow $P^* \in \Ps_{high}$),
using Lemma~\ref{lem:seg-prop} (3c), we claim that $\DE_0(P_1)$ and $\DE_0(P'_1)$ does not diverge after
intersecting.  Recall that in general this property is only satisfied by $\MD{P_1}$
(using Lemma~\ref{lem:ms-stdpath-prop}\ref{lem:ms-lastP0-interleave}) hence $\PP_b$ only handles the paths
with $|\MD{P_1}|>(n_\sigma)^{2/3}$.
%Here except for the cases where $P_1$ follows the
%representative paths of segments of $\PP_0$,
We can thus similarly bound the number of paths
with $|\DE_0(P_1)|>(n_\sigma)^{2/3}$ to $O(\sigma^{1/3}n^{2/3})$. Thus, we have the
following lemma.

\begin{lemma}
Except for $O(\sigma^{1/3}n^{2/3})$ paths in $\PP_c$, for any contributing path $P\in\PP_c$,
$P_1$ does not follow any representative path or any path in $\Ps_{high}$ and
$\DE_0(P_1)\leq (n_\sigma)^{2/3}$
\label{lem:ms-Pd-P1-prop}
\end{lemma}

We are now ready to apply Lemma~\ref{lem:seg-prop}, this time with different parameters.
Using Lemma~\ref{lem:ms-stdpath-prop}\ref{lem:ms-lastP0-interleave}, we know that for paths $P_1\in\PP_{1c}$,
the set of $\MD{P_1}$ forms a set of segmentable paths ($\Ps_*$).
Since we consider only those paths in $\PP_c$ which emerge from $\MD{P_1}$
(using Lemma~\ref{lem:ms-stdpath-prop}\ref{lem:ms-LP-nonLL0}),
the set of paths $\MD{P}$ for $P\in \PP_c$ starts from the same vertex as the corresponding $\MD{P_1}$.
Also, by definition of $\PP_c$, $\DE_0(P_1)$ does not intersect with $\Ps_{high}$ and $e_1\in \Ps_{high}$.
Thus, $\MD{P}$ is the shortest path from $\SC(\MD{P_1})$ to $v$ avoiding $e_2\in \MD{P_1}$.
Hence, for all $P\in \PP_c$, we can apply Lemma~\ref{lem:seg-prop} using $\Ps_*$ as the set $\{\MD{P_1} |\ P_1 \in \PP_{1c}\}$,
$\Ps$ as the set $\{\MD{P}\ |\ P \in \PP_c\}$, $\DE_*(P)$ as $\DE_1(P)$, and $e\in P_*$ as the corresponding $e_2\in P_1$.


Now, by definition every path in $\Pthr{\PP}{1}{c}$ we have $|\MD{P_1}|\leq n_\sigma^{2/3}$.
Thus, considering all sources the total number of paths in $\MD{P_1}$ for all $P_1\in \PP_{1c}$ are
$O(\sigma n_\sigma^{2/3})$. This also limits the number of segments of $\MD{P_1}$ to
$O(\sigma^{1/3} n^{2/3})$
(using Lemma~\ref{lem:seg-prop} (1)).
Since, two contributing paths enter $v$ using a unique edge, using Lemma~\ref{lem:seg-prop} (2) there will be
exactly one path in $\PP_c$ that follows the representative path.
Also, a contributing path in $\PP_{c}$ does not follow any
path in $\PP_{1c}$
(else such paths are non-contributing). Thus,  number
of
paths in $\PP_c$ that follow the representative path or
a path in $\PP_{1c}$  is limited to
$O(\sigma^{1/3}n^{2/3})$. Now, except for these $O(\sigma^{1/3}n^{2/3})$ paths, any two paths in $P,P'\in\PP_c$
also satisfies that $\DE_1(P)$ and $\DE_1(P')$ do not diverge if they intersect (using Lemma~\ref{lem:seg-prop}~3(c)).
Since, each path in $\PP_c$ is contributing it  enters $v$ from a unique edge,  $\DE_1(P)$ cannot intersect
with detour of any other path in $\PP_c$. Since remaining $\DE_1(P)$ are disjoint,
the number of such paths with $|\DE_1(P)|> (n_\sigma)^{1/3}$,
can  by restricted to $O(\sigma^{1/3}n^{2/3})$. Hence, for the remaining paths in $\PP_c$ we have
$|\DE_1(P)|<n_\sigma^{1/3}$ giving the following corollary.

\begin{lemma}
Except for $O(\sigma^{1/3}n^{2/3})$ paths in $\PP_c$, for any paths  $P\in\PP_c$ we have
$|\DE_1(P)|\leq n_\sigma^{1/3}$.
\label{lem:ms-Pd-short-detour}
\end{lemma}

We shall now bound the number of paths in $\PP_c$ to $O(\sigma^{1/3}n^{2/3})$.
Let $\PP'_c$ be the set of paths in $\PP_c$ removing $O(\sigma^{1/3}n^{2/3})$ paths described in
Lemma~\ref{lem:ms-Pd-P1-prop} and Lemma~\ref{lem:ms-Pd-short-detour}.
Let $\PP'_c(s)$ be the subset of paths in $\PP'_c$ that start from a source $s \in S$.
Also, let $\PP'_{1c}(s)$ be the corresponding $P_1$ for each $P\in \PP'_c(s)$.
Using Lemma~\ref{lem:ms-Pd-P1-prop} and Lemma~\ref{lem:ms-Pd-short-detour},
for any path $P\in \PP'_c$(s), we have $|\DE_0(P_1)| \le n_\sigma^{1/3}$ and
$|\DE_1(P)|\leq n_\sigma^{1/3}$.


For any path $P\in \PP'_c(s)$, we have
$|P|\geq P_0[s,v]$. Let $x=\SC(\DE_0(P_1))$ and $y=\SC(\DE_1(P))$.
Thus, $P$ can be divided into three parts  as follows.
\begin{align*}
        |P|     &=              |P[s,x]|+|P[x,y]|+|P[y,v]|\\
                        &=   |P_0[s,x]|+|\DE_0(P_1)[x,y]|+|\DE_1(P)[y,v]| &\qquad\text{(by definition of $x$ and $y$)}\\
                        &\leq   |P_0[s,v]|+|\DE_0(P_1)|+|\DE_1(P)|\leq |P_0[s,v]|+n_\sigma^{2/3}+n_\sigma^{1/3}
\end{align*}


Using Lemma~\ref{lem:stdpath-prop}\ref{lem:diffP}, we know that for any $P,P'\in \PP_c(s)$ we have $|P|\neq |P'|$.
We thus arrange the paths in $\PP'_c(s)$ in the increasing order of sizes,
where $i^{th}$ such path has the length $\geq |P_0[s,v]|+i$.
Hence, the maximum value of such $i$ is $O(n_\sigma^{2/3})$
limiting total number of such paths in $\PP'_c(s)$ to $O(n_\sigma^{2/3})$.
Thus the total number of paths in $\cup_s \PP'_c(s) = O(\sigma n_\sigma^{2/3}) = O(\sigma^{1/3}n^{2/3})$.
%Thus, we claim the following theorem
%\begin{theorem}
%        The number of contributing paths of the type $\PP_c$ are $O(\sigma^{1/3}n^{2/3})$.
%        \label{thm:ms-contPdD}
%\end{theorem}

